Improving Semantic Composition with Offset Inference

Count-based distributional semantic models suffer from sparsity due to unobserved but plausible co-occurrences in any text collection. This problem is amplified for models like Anchored Packed Trees (APTs), that take the grammatical type of a co-occurrence into account. We therefore introduce a novel form of distributional inference that exploits the rich type structure in APTs and infers missing data by the same mechanism that is used for semantic composition.

==> _tables/feature_space.tex <==
\begin{table*}[!htb]
\centering
\small
%\resizebox{\textwidth}{!}{
\begin{tabular}{ l | l || l }
\textbf{\APT~for \emph{white} - Features} & \textbf{\APT~for $\emph{white}^\texttt{amod}$ - Features} & \textbf{\APT~for \emph{clothes} - Features}\\ \hline
\texttt{:}\emph{clean} & \texttt{amod:}\emph{clean} & \texttt{amod:}\emph{wet} \\
%\texttt{:}\emph{black} & \texttt{amod:}\emph{black} & \texttt{amod:}\emph{black}  \\
\texttt{\textoverline{amod}:}\emph{shoes} & \texttt{:}\emph{shoes} & \texttt{:}\emph{dress} \\
%\texttt{\textoverline{amod}:}\emph{noise} & \texttt{:}\emph{noise} & \texttt{:}\emph{silk} \\
%\texttt{\textoverline{amod}.\textoverline{compound}:}\emph{silk} & \texttt{\textoverline{compound}:}\emph{silk} & \texttt{\textoverline{compound}:}\emph{silk} \\
%\texttt{\textoverline{amod}:\textoverline{compound}:}\emph{dress} & \texttt{\textoverline{compound}:}\emph{dress} & \texttt{\textoverline{compound}:}\emph{dress} \\
\texttt{\textoverline{amod}.\textoverline{dobj}:}\emph{wear} & \texttt{\textoverline{dobj}:}\emph{wear} & \texttt{\textoverline{dobj}:}\emph{wear} \\
%\texttt{\textoverline{amod}:\textoverline{dobj}:}\emph{prefer} & \texttt{\textoverline{dobj}:}\emph{prefer} & \texttt{\textoverline{dobj}:}\emph{appear} \\
%\texttt{\textoverline{amod}.\textoverline{nsubj}.}\emph{earn} & \texttt{\textoverline{nsubj}:}\emph{earn} & \texttt{\textoverline{nsubj}:}\emph{admit} \\
%\texttt{\textoverline{amod}:\textoverline{nsubj}:}\emph{own} & \texttt{\textoverline{nsubj}:}\emph{own} & \texttt{\textoverline{nsubj}:}\emph{appear} \\
\texttt{\textoverline{amod}.\textoverline{dobj}.nsubj:}\emph{coat} & \texttt{\textoverline{dobj}.nsubj:}\emph{coat} & \texttt{\textoverline{dobj}.nsubj:}\emph{actor}\\
%\texttt{\textoverline{amod}:\textoverline{dobj}:nsubj:}\emph{flower} & \texttt{\textoverline{dobj}:nsubj:}\emph{flower} &
\end{tabular}%}
\captionsetup{font=small}
\caption{Sample of vectorised features for the {\APT}s shown in Figure~\ref{apt_space}. Offsetting \emph{white} by \texttt{amod} creates an offset view, $\emph{white}^\texttt{amod}$, representing a noun, and has the consequence of aligning the feature space with \emph{clothes}.}
\label{apt_feature_space}
\end{table*}

==> background.tex <==
The basis of how composition is modelled in the {\APT}~framework is the way that the co-occurrences are structured. In characterising the distributional semantics of some lexeme $w$, rather than just recording that the lexeme $w^{\prime}$ co-occurred within some context window with $w$, following~\citet{Pado_2007}, the co-occurrence is typed, recording the dependency path from $w$ to $w^{\prime}$. This type information imposes a structure on the semantic space which makes it possible to precisely align the semantic representations of each of the lexemes being composed in some phrase. 

Many simple, yet very successful approaches to modelling semantic composition, such as pointwise vector addition or multiplication, neglect the structural information of the text and therefore lose information in the composition process. This subsequently results in the fundamental problem that composition is a fully commutative operation, which is undesirable for many natural language understanding problems. 

{\APT}s avoid the commutativity problem by leveraging the syntactic structure of a given phrase, giving rise to very diverse feature spaces between lexemes with different parts of speech. For example many nouns will have distributional features starting with the type \texttt{amod}, which cannot be observed for adjectives or verbs. Thus, when composing the adjective \emph{white} with the noun \emph{clothes}, the feature spaces of the two lexemes need to be aligned first. This can be achieved by offsetting one of the constituents, which we will explain in more detail in the next section. 

We will make use of the following notation throughout this work. A typed distributional feature consists of a path and a lexeme such as in the adjectival feature \texttt{amod:}\emph{white} for a given noun. Inverse paths are denoted by a horizontal bar above the dependency relation such as in the feature \texttt{\textoverline{dobj}:}\emph{prefer}. We separate higher-order paths with a dot such as in the feature \texttt{\textoverline{amod}.\textoverline{compound}:}\emph{dress}. The offset view of a given lexeme for a given path is denoted by superscripting the offset path, for example the \texttt{amod} offset of the adjective \emph{white} will be denoted as $\emph{white}^\texttt{amod}$.
